Implementing Strassen's Algorithm with CUTLASS on NVIDIA Volta GPUs

Conventional GPU implementations of Strassen's algorithm (Strassen) typically rely on the existing high-performance matrix multiplication (GEMM), trading space for time. As a result, such approaches can only achieve practical speedup for relatively large, "squarish" matrices due to the extra memory overhead, and their usages are limited due to the considerable workspace. We present novel Strassen primitives for GPUs that can be composed to generate a family of Strassen algorithms. Our algorithms utilize both the memory and thread hierarchies on GPUs, reusing shared memory and register files inherited from GEMM, fusing additional operations, and avoiding extra workspace. We further exploit intra- and inter-kernel parallelism by batching, streaming, and employing atomic operations. We also develop a performance model for NVIDIA Volta GPUs to select the appropriate blocking parameters and predict the performance for GEMM and Strassen. Overall, our 1-level Strassen can achieve up to 1.11x speedup with a crossover point as small as 1,536 compared to cublasSgemm on a NVIDIA Tesla V100 GPU. With additional workspace, our 2-level Strassen can achieve 1.19x speedup with a crossover point at 7,680.

==> acknowledgment.tex <==

The numerical simulations needed for this work were performed on Microway's Tesla GPU accelerated compute cluster. The authors are grateful for the HPC time provided by Microway, Inc.



==> analysis.tex <==

%\input module_analysis

\input model

%\begin{figure}[h]
%  \centering \includegraphics[scale=.3]{figures/analysis.pdf} 
%pdf\caption{\small 
%small}
%  \label{fig:analysis}
%\end{figure}

%\textbf{Time breakdown:}




==> impl.tex <==



\subsection{Exploiting more parallelism}
\label{s:parallel_gpu}
%inter-block and intra-block streaming
% what is the existing parallelism
A straightforward implementation of Strassen's algorithm based on our specialized kernel (\secref{s:gpu_stra}) would invoke a sequence of kernels sequentially
(7 kernels for one level, 49 kernels for two levels).
%intra-kernel vs. inter-kernel parallelism
%utilize GEMM implementation to achieve inter-block parallelism.
This approach has already achieved the intra-kernel parallelism across the thread blocks, warps, and threads,
which is utilized in the \gemm{} implementation on a GPU.
% However, Challenges: more levels need more parallelism
However, it is further possible to improve concurrency by
exploiting more inter-kernel parallelism.
A careful observation of
%\figref{fig:gpu_strassenlevel1}
\eref{eqn:gpu_allops}
reveals that
\begin{itemize}
    \item the ordering of these operations can be arbitrary;
    \item the dependencies between the kernels for these operations only occur for the concurrent writes to different submatrices of $ C $.
\end{itemize}
% more important for
% - multi-level Strassen
% - small problem sizes, when un saturated.
By invoking multiple independent kernels without write dependencies to different parts of $ C $, we can achieve inter-kernel parallelism, which is especially important for small problem sizes when there is limited intra-kernel parallelism such that each kernel cannot saturate the workload for the GPU device and for multi-level \strassen{} when the partitioned block size is small.
%However, 7 blocks
%7 operations in equation () are totally independent, if we ignore the parts for writing C.
We exploit the inter-kernel parallelism in the following ways:
%\begin{itemize}
\subsubsection*{Multi-kernel streaming}
    %What is stream
    CUDA programs can manage the concurrency across kernels through \emph{streams}~\cite{cuda}, each of which is a sequence of commands that execute in order.
    While the instructions within the same stream must be scheduled in sequential order, the commands from different streams may run concurrently out of order.
    % with respect to each other or concurrently.
    %What is the benefit of stream
    This helps to overlap computation with communication, as well as run multiple kernels at the same time.
    To ensure every command in a particular stream has finished execution, {\tt cudaDeviceSynchronize} can be used to enforce synchronization points.

    \tabref{tab:gpu_streaming} illustrates the multi-kernel streaming implementation with the reordered operations based on
%    \figref{fig:gpu_strassenlevel1}.
\eref{eqn:gpu_allops}.
    We organize the kernels for these operations into three stages with two streams.
    Synchronization of the streams is imposed between the different stages to guarantee the correctness of the operations because of the concurrent write dependencies to different parts of $ C $. The kernels for these operations in different streams within the same stage can be interleaved or executed concurrently.
    We note that \cite{StrassenGPU2} also leverage multi-kernel streaming to make use of concurrency across kernels for the bottom level \strassen{}. However, it requires an additional workspace of 15 extra submatrices, while our approach doesn't require any additional workspace due to our specialized kernels.
    \input table_streaming
    \subsubsection*{Element-wise atomic write to $ C $}
    Since the dependencies across the kernels only exist during the concurrent write to different parts of $ C $,
    we can ``partially'' remove the dependencies and execute all operations fully concurrently in one stage with one operation per stream
    by replacing the post-processing step\footnote{The post-processing step involves loading each element of $ D $ and $ E $ in the global memory, adding or subtracting corresponding element in $ M_i $ residing in the $ C $ \emph{Accumulator} in the register, and storing back to the original location of $ D $ and $ E $ in the global memory.} of submatrices of $ C $ 
    with element-wise atomic write operation through {\tt atomicAdd}.
    We find that this way will benefit small problem sizes. However, when the problem sizes become larger, 
    the performance drops because element-wise atomic operations
    incur a greater overhead.
    %cause much bigger overhead.

    \subsubsection*{Atomic write to $ C $ with larger granularity}
    Each thread finally updates an $ m_R \times n_R $ block of $ C $, so it is possible to switch the granularity of atomic write from $ 1 $ (element-wise) to $ m_R \times n_R $ (block-wise). We need to construct a device array for the purpose of a mutex/lock. Each entry of the device array corresponds to an $ m_R \times n_R $ block of $ C $.
Once a thread completes the accumulation of the $ C $ \emph{Accumulator} in the register, it will first lock the corresponding mutex/lock entries of $ m_R \times n_R $ block of $ D $ and $ E $ (different submatrices of $ C $) before updating $ D $ and $ E $, and unlock the corresponding mutex/lock entries after the updates finish. The locks can be implemented with {\tt atomicCAS} and {\tt atomicExch} functions.
%%%%%% The space for this mutex/lock array can be ignored....

    %dynamic scheduling
    %wait, signal
    \subsubsection*{Reducing the multi-kernel launch overhead}
    With the multi-kernel streaming, we still need to launch seven kernels for one-level \strassen{}.
For small problem sizes, the overhead for launching multiple kernels cannot be ignored. %may be non-negligible.
To further reduce the overhead for kernel launching and avoid the possible inefficiency caused by the CUDA stream implementation,
it is possible to just launch one kernel for all operations shown in
%\figref{fig:gpu_strassenlevel1}
\eref{eqn:gpu_allops}
with a 3-D grid of thread blocks,
while the \gemm{} and specialized kernels in
%\figsref{fig:gpu_gemm} and \ref{fig:gpu_stra}
\figref{fig:gpu_side_by_side}
only require a 2-D grid.
The additional $z$ dimension for the grid ({\tt blockIdx.z}) corresponds to different operations in
%\figref{fig:gpu_strassenlevel1}.
\eref{eqn:gpu_allops}.
The inter-kernel parallelism for multi-kernel streaming has thus transformed into one extra dimensional concurrency inside the kernel.
We can use atomic write with the granularity of either 1 or $ m_R \times n_R $ to guarantee the correctness of the result.

%%%%%% Measure the overhead of kernel launching
% compare the performance of 
% multi-kernel launching ( 2 streams )
% multi-kernel launching ( 7 streams ), atomic write
% multi-kernel launching ( 7 streams ), atomic write with mutex
% one 3-D launching, atomic write
% one 3-D launching, atomic write with mutex
%%%%%%

\subsection{Reducing memory requirement}

The conventional implementations of \strassen{} on GPUs based on the functions provided by cuBLAS for matrix multiplication and matrix addition (i.e., {\tt cublasSgemm, cublasSgeam}) led to the ``street wisdom'' that there is a 
trade-off between reducing the effective available memory and exploiting more parallelism.
%More parallelism traditionally requires to have
More temporary workspace for intermediate result is traditionally required to eliminate the dependency and increase the concurrency.
With our approach, however, we can achieve both reduced memory and more homogeneous parallelism, similar to data parallelism except the dependencies for concurrent writes to different parts of $ C $. We reuse the shared memory to store the temporary sum and the register file to store the temporary matrix product $ M_i $ (\secref{s:gpu_stra}). The different operations in
%\figref{fig:gpu_strassenlevel1}
\eref{eqn:gpu_allops}
can be easily parallelized with the help of multi-kernel streaming or one kernel with a 3-D grid (\secref{s:parallel_gpu}).

%% Benefit of our approach
%With our approach, we can achieve both.
%packing and accumulating update reuse the memory, save workspace requirement

%{packing}
%vector load?
%vector store?
%lds.128
%ldg.128
%register consumption
%%\subsubsection*{rank-$1$ update kernel}
%{updating accumulator}
%write from the kernel directly

\subsection{Handling the fringes}

Traditionally, for matrices with odd dimensions, we need to handle the remaining fringes before applying \strassen{}.
There are some well-known approaches such as padding (i.e., adding rows or columns with zeros to get matrices of even dimensions) and
peeling (i.e., deleting rows or columns to obtain even dimensioned matrices)~\cite{Huss-Lederman:1996:ISA:369028.369096, StrassenDynamicPeeling}
followed by post-processing.
In our approach, fringes can be internally handled by padding the $ A $ \emph{Tile} and $ B $ \emph{Tile} with zeros,
and aligning the $ m_C \times n_C $ $ C $ \emph{Accumulator} along the fringes.
This trick avoids the handling of the fringes with extra memory or computations because the packing and accumulation processes always occur for
high-performance implementation of \gemm{} on GPUs, and we reuse the same buffers.
% alighment? always aligned?

\subsection{Adapting software prefetching}

As illustrated in \algthmref{a:gpu_stra}, instead of prefetching one $ m_S \times k_S $ block of $ A $ and one $ k_S \times n_S $ block of $ B $,
%we now need to preload
\strassen{} requires the preloading of
two $ m_S \times k_S $ blocks of $ X $ and $ Y $ and two $ k_S \times n_S $ blocks of $ V $ and $ W $.
The required register number per thread has since doubled, but the required sizes of shared memory and global memory remain the same.

\input alg_stra




\subsection{Variants}

\begin{itemize}
    \item ABC
    \item XXC 
    \item XXX
\end{itemize}

composition of these variants.

C - ABC variants.





% \cite{StrassenGPU2}
% at each level of Strassen, the matrix is divided into multiple sub-matrices for computation.
% at the bottom level, it has the smallest sized matrix for computation and provides a good opportunity to take advantage of multi-kernel streaming on GPU.:w


\subsection{Performance model}

\cite{GPUmodel1}
\cite{GPUmodel2}

\begin{figure}[htp!]
\center
\input figures/model_square_perf_V100_SXM2
\caption{
    Comparison of different modules.
}
\label{fig:model_square}
\end{figure}




\subsection{Numerical stability}


7 operations, 4 streams:
49 operations, 10 streams:

